HARNESS: Lightweight Distilled Arabic Speech Foundation Models

Large self-supervised speech (SSL) models achieve strong downstream performance, but their size limits deployment in resource-constrained settings. We present HArnESS, an Arabic-centric self-supervised speech model family trained from scratch with iterative self-distillation, together with lightweight student variants that offer strong accuracy-efficiency trade-offs on Automatic Speech Recognition (ASR), Dialect Identification (DID), and Speech Emotion Recognition (SER). Our approach begins with a large bilingual Arabic-English teacher and progressively distills its knowledge into compressed student models while preserving Arabic-relevant acoustic and paralinguistic representations. We further study PCA-based compression of the teacher supervision signal to better match the capacity of shallow and thin students. Compared with HuBERT and XLS-R, HArnESS consistently improves performance on Arabic downstream tasks, while the compressed models remain competitive under substantial structural reduction. These results position HArnESS as a practical and accessible Arabic-centric SSL foundation for real-world speech applications.

==> Sections/harness_model.tex <==
Figure \ref{fig:overview} gives an overview of the HArnESS training pipeline, which follows a HuBERT-style iterative self-distillation approach.

\noindent\textbf{Training Regimen} At each iteration $i$, we train a model $\mathbf{M}_{i}$ using the pseudo-labels from the previous $(i-1)$ iteration model as supervisory signals. 
% We obtained these pseudo-labels by clustering the $(i-1)$ model's hidden representation. 
The model then learns to classify randomly masked frames to these pseudo-labels. 
In the first two iterations, we retain the same architecture to enhance feature abstraction in the student model. From the third iteration, we compress the model through distillation by: \textit{(a)} reducing depth ($d$) for a shallower architecture; \textit{(b)} reducing width ($enc_d$) for a thinner model, and
\textit{(c)} lowering attention capacity ($attn$) by decreasing attention heads.
% Moreover, we also explore the performance effect lowering attention capacity ($attn$) .
% For the first two iterations, we maintain the same model architecture to ensure improved feature abstraction in the student. However, from the third iteration onward, we reduced the model size through distillation by: (a) making the architecture shallow -- reducing the model depth ($d$); (b) making it thinner -- reducing model width (encoder dimension, $enc_d$); and/or reducing attention capacity ($attn$) bylowering the number of attention heads. 


\noindent\textbf{Model Architecture}
The HArnESS model consists of a convolutional (CNN) feature extractor and Transformer encoders. Similar to HuBERT, WavLM \cite{chen2022wavlm} and Wav2Vec2.0 \cite{baevski2020wav2vec}, the CNN feature extractor includes 7 temporal convolution layers. The transformer encoder layers $l$ have embedding dimension $enc_d$, and are composed of a multi-head self-attention (MHA) with $attn$ heads and a position-wise feed-forward network (FFN).

\noindent\textbf{Training Objectives} We use the weighted sum of two cross-entropy losses, applied separately to the masked and unmasked frames as training objectives.
% The objective of the model, at $iter=i$ is to predict randomly masked frames to pseudo labels, generated by custering the $iter=i-1$ model's output embeddings.  


\noindent\textbf{Weight Initialization} We explored different weight initialization strategies to improve convergence and stability. We experimented with random weight initialization, where model weights were initialized using a uniform random distribution to introduce diversity in parameter values at the start of training. Additionally, we also employed a blocked averaging initialization approach, where weights were initialized by averaging blocks of layers from the preceding model. 
% This method facilitated a smoother transition between iterations, helping to retain learned representations while enabling progressive refinement.

\noindent\textbf{Pseudo-labels generation} 
We employ K-means clustering to assign discrete labels to speech frames, leveraging last-layer embeddings, which capture the most refined high-level representations from the model.\footnote{We also explored averaged embeddings from selected layers but found no significant differences.} 
% To enhance clustering efficiency for distillation, we apply Principal Component Analysis (PCA) to filter out redundant information and retain only the most meaningful features for representation.
Before clustering, we apply Principal Component Analysis (PCA) to reduce the dimensionality of these dense embedding features. PCA is a statistical procedure that orthogonally transforms the high-dimensional embeddings into a set of linearly uncorrelated variables, ordered by their variance. We introduce PCA in this pipeline for two critical reasons. First, it mitigates the curse of dimensionality, which degrades distance metrics like Euclidean distance used in K-means, while filtering out spurious noise by retaining only the most salient acoustic variances. Second, and crucially for deployment in resource-limited environments, compressing the dimensionality of the teacher's representations facilitates our model compression strategy. By mapping the dense features to a lower-dimensional space, we are able to effectively train a student architecture with a significantly reduced hidden dimension size ($emb_{d}$). This architectural reduction in $emb_{d}$ directly and substantially decreases the total parameter count of the student model.
% We generated discrete pseudo-labels that served as supervisory signals for training in subsequent iterations.
For the initial iteration, $i=0$, we initialize training by extracting MFCC features from the raw speech input $x$ and use them to generate the initial pseudo-labels. 

==> Sections/introduction_old.tex <==

Self-supervised learning (SSL) has revolutionized speech processing by extracting and learning transferable representations from large amounts of unlabeled speech. These large SSL models capture rich speech representations, making them highly effective across a wide range of speech-related tasks \cite{chen2022wavlm, hsu2021hubert,baevski2022data2vec,mohamed2022self,chung2021w2v,yang2021superbspeechprocessinguniversal}. These models can be leveraged either as feature extractors or fine-tuned with a small amount of labeled data, significantly improving performance in low-resource settings.

However, the generalization capability of SSL models is highly dependent on the diversity and volume of training data. Multilingual SSL speech models such as XLS-R \cite{babu2021xlsr} have demonstrated superior performance in low-resource languages compared to monolingual models, particularly those trained in high-resource languages like English \cite{shi2023mlsuperbmultilingualspeechuniversal}. Yet, recent findings by \cite{storey2024language} indicate that models like XLS-R tend to prioritize languages with abundant training data, potentially leading to suboptimal performance for underrepresented languages. This suggests that relying solely on multilingual models may not ensure optimal performance across all languages, and language-specific SSL models could be essential to address this gap effectively.


The \textbf{Arabic} language poses a unique challenge in speech processing due to its vast linguistic diversity. Spoken across 22 countries, Arabic includes more than 20 mutually incomprehensible dialects, with significant influences from other languages such as English and French \cite{ali_connecting_2021}. 
% The dialects spoken in North African regions (e.g., Morocco, Algeria, Tunisia) are particularly heavily influenced by French, while Levantine and Gulf dialects exhibit distinct phonetic, morphological, and syntactic variations.
Given this linguistic complexity, choosing an appropriate SSL model for Arabic speech tasks requires a model that can effectively capture the nuances of spoken dialects while preserving cultural and phonetic diversity. Multilingual models, though useful, may not fully grasp the intricacies of Arabic speech, making the case for a dedicated Arabic-English SSL model.
% 
However, training and deploying language-specific speech SSL models requires significant computational resources, large-scale unlabeled data, and prolonged training times, making them costly and inaccessible for many researchers. 
These high resource demands hinder efficient fine-tuning and deployment in resource-constrained settings.
% In practical -- resource-constrained settings, their high latency and resource demands further hinder efficient deployment and fine-tuning
% However, training language-specific speech SSL models demands extensive computational resources and huge amounts of unlabeled data, making them costly and time-consuming. This limits accessibility for academic researchers, hindering exploration.

% language-specific speech SSL models requires significant computational resources, as they rely on massive amounts of unlabeled speech data for effective pretraining before the fine-tuning. The high resource consumption and prolonged training times make these models inaccessible to many academic researchers, posing a significant barrier to explore these models.
% However, training language-specific speech SSL models demands enormous computational resources due to the need for massive quantities of unlabeled data, for effective pre-training before fine-tuning. 
% The extensive memory usage and prolonged training time of these models make them inaccessible to most researchers, contradicting the fast- paced demands of the AI industry.



% Moreover, in real-world applications or resource-constrained environments, deploying and fine-tuning these large speech SSL models can be computationally expensive and inefficient due to their high latency and resource demands. 
\textbf{Knowledge distillation} has emerged as a key technique for compressing large models while preserving their performance. Distillation enables a smaller, more efficient model (student) to learn from a larger, computationally expensive teacher model, reducing memory usage and inference time without significant performance degradation.
Early works such as DistillHuBERT \cite{chang2022distilhubert}, FitHuBERT \cite{lee2022fithubert}, DPHuBERT \cite{peng2023dphubert}, SKILL \cite{zampierin2024skill} among others \cite{ashihara2022deep,wang2022lighthubert} have applied task-agnostic knowledge distillation to HuBERT \cite{hsu2021hubert}.
% }, focusing on general-purpose model compression. 
% DPHuBERT \cite{} further explored structured pruning guided by distillation, optimizing model size without relying on task-specific data. More recently, SKILL \cite{} introduced a layer-wise similarity-based approach, where distillation is applied across groups of layers within the teacher model. 


While prior work has adapted self-supervised speech models such as HuBERT and wav2vec 2.0 to Arabic, Arabic-centric SSL remains underexplored, particularly for training from scratch at scale and for systematic compression into lightweight deployment-oriented models. In this work, we focus on these two aspects. We train an Arabic-centric SSL family, \textbf{H}uBERT-based \textbf{Ar}abic a\textbf{n}d \textbf{E}nglish \textbf{S}elf-\textbf{S}upervised Speech (HArnESS) model, from scratch using large-scale bilingual Arabic-English speech, and we study iterative self-distillation to produce compact students that retain strong performance across ASR, SER, and DID.

% In this study, we introduce \textbf{H}uBERT-based \textbf{Ar}abic a\textbf{n}d \textbf{E}nglish \textbf{S}elf-\textbf{S}upervised Speech (HArnESS) models, the first family of Arabic self-supervised speech models, jointly trained on large-scale Arabic and English speech data from scratch. By training specifically on Arabic and English, HArnESS ensures better adaptation to dialectal variations and phonetic intricacies, making it a suitable choice for Arabic speech applications. 

% The HArnESS models are trained using iterative self-distillation, following the HuBERT architecture. 
% Our approach refines and enhances model performance by leveraging its own predictions as supervisory signals across multiple training iterations. This approach enables scaling model in a self-supervised manner by generating new pseudo-labels through clustering applied to the hidden layer outputs of previous iterations. 
% This approach enhances model performance by using its own predecessor's predictions as supervisory signals across multiple training iterations. 
% The process enables self-supervised scaling, where new pseudo-labels are generated through clustering on hidden layer outputs from previous iterations. 
% By repeating this process iteratively, the model gradually improves its encoded representations, leading to richer and more structured speech features.
We leverage this learning paradigm and train HArnESS-L with 24 encoder layers in the first few iterations, preserving its deep architecture. In the following iteration, we distill its knowledge into lightweight student models, resulting in HArnESS-S (shallow) and HArnESS-ST (shallow and thin) architectures. 
Furthermore, we apply low-rank approximation to compact the supervisory signal with rich and informative representation and ensure efficient and fast knowledge transfer.

We adopt bilingual Arabic-English pretraining for two reasons. First, English corpora provide additional acoustic and phonetic diversity at scale, which can stabilize self-supervised representation learning when Arabic resources are comparatively limited and heterogeneous. Second, Arabic speech in real-world settings often co-occurs with borrowed English words and code-switching, especially in conversational and media speech. Our goal is therefore not to dilute Arabic-specific modeling, but to combine Arabic-centric coverage with the regularization benefits of broader bilingual pretraining.

% We leverage this learning paradigm, with inital iterations learning and distilling knowledge in similar architecture (depth of 24 encoder layers: HArnESS-L), and then on the subsequent iteration, we distill knowledge from the HArnESS-L to several lightweight students with shallow (HArnESS-S) and thin (HArnESS-ST) architectures. 
% Hence, we exploit the preceding iteration of the large teacher model to transfer richer gradients to the smaller SSL models.
% we exploit the preceding iteration of large model to transfer richer gradients to the small scale SSL models. 
% NOT SURE!!
% Additionally, we apply low-rank approximation to compress the student model while distilling knowledge from the teacher model. This allows us to reduce the feature dimension of the teacher while maintaining essential speech representations, making the smaller models more efficient for downstream tasks.

% we compressed the student model and distilled knowledge from the teacher model by applying low-rank approximation to reduce feature dimension of the teacher.  

We evaluated the HArnESS-L, HArnESS-S, and HArnESS-ST models on downstream tasks including Automatic Speech Recognition (ASR), Speaker emotion recognition (SER), and Dialect identification (DID). We also compared the performance of these models with HuBERT-large (English)  and XLS-R (multilingual) \cite{babu2021xlsr} models.

% \begin{figure*}[!ht]
%     \begin{center}   
%     \includegraphics[scale=0.85]{LREC2026/figures/Overview2.png}        
%     \caption{Overview: Iterative self-distillation training to build HArnESS model family.}
%     \label{fig:overview}
%     \end{center}
% \end{figure*}

\begin{figure*}[!ht]
    \begin{center}   
    \includegraphics[scale=0.5]{LREC2026/figures/HArnESS-2.png}        
    \caption{Overview: Iterative self-distillation training to build the HArnESS model family.}
    \label{fig:overview}
    \end{center}
\end{figure*}


\noindent Therefore, our key contributions are:
\begin{enumerate}
    \item Introducing HArnESS, the first Arabic-centric self-supervised speech model family with HArnESS-L (large), HArnESS-S (shallow), and HArnESS-ST (shallow and thin) architectures, trained from scratch.
    \item Exploring the iterative self-distillation paradigm for Arabic model compression and knowledge distillation.
    \item Investigating the effect of compact supervision signals on model performance. 
    \item Publicly releasing distilled models (HArnESS-S and HArnESS-ST) for research.\footnote{Links removed for anonymity.}
    \item Benchmarking HArnESS on content (ASR), speaker information (DID), and paralinguistic (SER) tasks. 
    \item Releasing benchmark datasets to support further research.\footnotemark[1]
    
\end{enumerate}
